Meta Learning for Natural Language Processing: A Survey

Deep learning has been the mainstream technique in natural language processing (NLP) area. However, the techniques require many labeled data and are less generalizable across domains. Meta-learning is an arising field in machine learning studying approaches to learn better learning algorithms. Approaches aim at improving algorithms in various aspects, including data efficiency and generalizability. Efficacy of approaches has been shown in many NLP tasks, but there is no systematic survey of these approaches in NLP, which hinders more researchers from joining the field. Our goal with this survey paper is to offer researchers pointers to relevant meta-learning works in NLP and attract more attention from the NLP community to drive future innovation. This paper first introduces the general concepts of meta-learning and the common approaches. Then we summarize task construction settings and application of meta-learning for various NLP problems and review the development of meta-learning in NLP community.

==> backup.tex <==
%Hung-yi Lee: I put some random draft below.
\subsection{Learn to Life-long learning} \label{subsec: learn_to_lifelong} %(Hung-yi)
In this section, we will talk about how to use meta learning to improve life-long learning.
The real world is changing and evolving from time to time, and therefore machines naturally need to update and adapt to the new data they receive.
However, when a trained deep neural network is adapted to a new dataset with a different distribution, it often loses the knowledge previously acquired and performs the previous task worse than before.
This phenomenon is called \textit{catastrophic forgetting}~\cite{Mccloskey89-catastrophic}.

Life-long learning is critical even though multiple diverse tasks are not considered. 
Just like humans, artificial neural networks sometimes make mistakes.
A single model error can lead to devastating financial, reputational, and even life-threatening consequences in many applications. 
Therefore, it is essential to correct model mistakes quickly as they appear. 
Since mistakes are inevitable, deep learning practitioners should be able to adjust model behavior by correcting errors as they appear. 
However, this is often difficult due to the nature of deep neural networks. 
In most network architectures, a prediction for a single input depends on all model parameters. Therefore, updating a neural network to change its predictions on a single input can decrease
performance across other inputs.
The research about developing reliable and computationally efficient methods for network bug-fixing is neural network editing − how one can efficiently patch a mistake of the model on a particular sample without influencing the model behavior on other samples.
Neural network editing can be considered as one scenario of life-long learning. 

%general solution %https://www.overleaf.com/project/60b78f641cdddc808e76e683
Re-training the models from scratch with both the past and the new data jointly, sometimes referred to as \textit{multitask learning}, is one very effective way to deal with catastrophic forgetting.
For various reasons, including privacy issues and the limited storage capacity, the earlier data are unlikely to be kept forever.
Therefore, \textit{lifelong learning} (LLL) or \textit{continual learning} \cite{Chen18-llml}, aiming for training a single model to perform a stream of tasks without forgetting those learned earlier, not relying on keeping all training data from the beginning, becomes a necessary goal for the continuously changing real world.
In general, LLL approaches can be categorized into the following types.
Regularization-based methods aim to consolidate essential parameters in a model by adding regularization terms in the loss function \cite{Kirkpatrick17-ewc, Schwarz18-online-ewc, Zenke17-si, Aljundi18-mas, Ehret20-rnn-hypernet}.
%Architecture-based methods try to assign some model capacity for each task or expand the model size to handle additional tasks \cite{Rusu16-progressive, Fernando17-pathnet, Mallya18-packnet}.
Data-based methods try to save or generate some samples from the past tasks to prevent catastrophic forgetting \cite{Lopez17-gem, Li17-lwf, Sun19-lamol, Von19-hnet, Saha21-gpm}.

%Studies of LLL have been reported more on computer vision \cite{Kirkpatrick17-ewc, Zenke17-si, Aljundi18-mas, Ehret20-rnn-hypernet,Fernando17-pathnet, Mallya18-packnet, Lopez17-gem, Li17-lwf, Von19-hypernet, Benavides20-knowlll, Mendez20-compositional, Wen20-batchensemble, Von19-hnet, Saha21-gpm} and reinforcement learning \cite{Kirkpatrick17-ewc, Schwarz18-online-ewc, Rusu16-progressive, Fernando17-pathnet, Rostami20-task-descript}, yet much less on automatic speech recognition (ASR) tasks \cite{Xue19-mtl-asr, Sadhu20-continual, Houston20-continual, Fu20-incremental}.

\subsubsection{Meta Learning for Regularization-based methods}

The work~\citet{sinitsin2020editing} presents an alternative approach that we call Editable Training. This approach involves training neural networks in such a way that the trained parameters can be easily edited afterwards. Editable Training employs modern meta-learning techniques (Finn et al. (2017)) to ensure that model’s mistakes can be corrected without harming its overall performance. It empirically demonstrates the effectiveness of this method on machine translation tasks.


The paper presents KnowledgeEditor~\citet{decao2021editing}, a method that can be used to edit this knowledge and, thus, fix 'bugs' or unexpected predictions without the need for expensive re-training or fine-tuning. 
The approach treats editing a neural model as a learning-to-update problem. 
It uses an efficient parameterization of a hyper-network that is trained to update the model parameters when provided with new data to edit network. 
The approach constrains the edited model to retain the same predictions as the original one regardless of the distance between the original and updated models in the parameter space. 
The hyper-network can be regarded as a 'probe' revealing which components of the network need to
be changed to manipulate factual knowledge, i.e., revealing the 'causal mediation mechanisms' (Vig et al., 2020).

%Unlike conventional Knowledge Bases (KBs) that explicitly store factual knowledge, neural models implicitly memorize facts in their parameters. One cannot easily access and interpret their computation and memories (Ribeiro et al., 2016; Belinkov and Glass, 2019; Voita et al., 2019; De Cao et al., 2020), thus, modifying their knowledge is a challenging problem.

\subsubsection{Meta Learning for Data-based methods}

A successful way to achieve lifelong learning is to enhance the model learning with an episodic memory module (Sprechmann et al., 2018).
The basic idea is to first store a limited number of previously seen training examples in memory, and then use them to perform empirical replay (Rolnick et al., 2019) or to derive optimization constraints (Lopez-Paz and Ranzato, 2017; Chaudhry et al. Human al., 2019).
Recently, d'Autume et al. (2019) proposes to use such a memory module for experience replay and apply local adaptation in NLP tasks, including text classification and QA.
%However, the data-based approahces have three significant impediments: (1) needing unrealistically large memory module to achieve good performance, (2) suffering from negative transfer, (3) requiring multiple local adaptation steps for each test example that significantly slows down the inference speed. 

\citet{wang-etal-2020-efficient} 
Meta learning can decrease the number of training examples in memory.
In order to achieve sample efficiency, the previous method trains the model in a way to learn better local adaptation initialization.
The experiments on text classification and QA benchmarks have verified the effectiveness of the framework, using only 1\% of the memory size to achieve the most advanced performance.

\citet{obamuyide-vlachos-2019-meta} \citet{wu2021meta-lifelong-re} 
Most existing relation extraction models assume a fixed set of relations. It is necessary to develop methods that enable the relation extraction model to continuously adapt and learn. Continuous relationship extraction is an important task, and the focus is on incrementally extracting new facts from unstructured text. Given the relation sequence, this task is prone to face two serious challenges, catastrophic forgetting and sequence sensitivity.

%However, given the continuous and iterative nature of the update process, continual relation extraction (Wang et al. 2019;Obamuyide and Vlachos 2019) is a more realistic and useful setting. Yet due to the limitations of storage and computational resources, it is impractical to grant the relation extractor access to all the training instances in previously seen tasks. Thus, this continual learning formulation is in contrast to the conventional relation extraction setting where the extractor is generally trained from scratch with the full access to the training corpus. Continual relation extraction is an important task that focuses on extracting new facts incrementally from unstructured text. Given the sequential arrival order of the relations, this task is prone to two serious challenges, namely catastrophic forgetting and order-sensitivity.


%The previous work propose a novel curriculum-meta learning method to tackle the above two challenges in continual relation extraction. We combine meta learning and curriculum learning to quickly adapt model parameters to a new task and to reduce interference of previously seen tasks on the current task. We design a novel relation representation learning method through the distribution of domain and range types of relations. Such representations are utilized to quantify the difficulty of tasks for the construction of curricula. Moreover, we also present novel difficulty-based metrics to quantitatively measure the extent of order-sensitivity of a given model, suggesting new ways to evaluate model robustness. Our comprehensive experiments on three benchmark datasets show that our proposed method outperforms the state-of-the-art techniques.

%EAEMR (Wang et al. 2019) proposes a sentence embedding alignment mechanism in memory maintenance and adopt it to continual relation extraction learning. Based on EA-EMR, MLLRE (Obamuyide and Vlachos 2019) introduces a metalearning framework for fast adaptation and EMAR (Han et al. 2020a) introduces a multi-turn co-training procedure
%for memory-consolidation. Most of these methods explore
%CF problem in the overall performance of task sequences,
%but they lack the insight analysis of the characteristics of
%each subtask and the corresponding model performance.


In meta learning, usually, we assume stationary task distribution. 
Can we do meta learning with evident distributional shift or when datasets arriving sequentially?
There is also research along the direciton~\cite{yap2021onlinemeta,finn20191onlinemeta}, but out of the scope of this subsection.

%Hung-yi Lee: I put some random draft below.
\subsection{Learn to Generalize} \label{subsec: learn_to_transfer}  %(Hung-yi) %Generalize? or transfer?

Traditional supervised learning assumes that the training and test data come from the same distribution. Domain shift refers to the problem that a model trained in a source domain performs poorly when applied to a target domain with different statistics. Domain generalization technology attempts to alleviate this problem by training models that can be well designed to generalize to new test domains. 

Domain generalization is also an important research topic of NLP.
Recently, pre-training large-scale LM and fine-tuning downstream labeled data is one way to improve domain generalization.
For example, by pre-training a multilingual LM on multilingual data, a model fine-tunes by one language's labeled data can be extended to multiple languages.
Multilingual pre-training language model methods usually involve two problems~\citep{li-etal-2020-learn}: (1) simply fine-tuning may not adapt general-purpose multilingual representations to be task-aware on low-resource languages; (2) ignore how cross-lingual adaptation happens for downstream tasks. 
On the other hand, the existing pre-training model adaptation method does not consider the result on new domains after fine-tuning.
Can meta-learning help the model learn to generalize?

%Domain Adaptation: Use little data from target domain to adapt. This is a few-shot learning problem. It is intuitive to apply meta learning here.
%Training models that generalize to new domains at test time is a problem of fundamental importance in machine learning.
%Domain Generalization:  Domain Generalization (DG) techniques attempt to alleviate this issue by producing models which by design generalize well to novel testing domains. The training data may include multiple domains. But we know nothing about the target domain. How to use meta learning to improve domain generalization?

%Below are approaches for CV, not NLP
\begin{comment}
\citet{li2018metaDG} We propose a novel {meta-learning} method for domain generalization. Rather than designing a specific model that is robust to domain shift as in most previous DG work, we propose a model agnostic training procedure for DG. Our algorithm simulates train/test domain shift during training by synthesizing virtual testing domains within each mini-batch. The meta-optimization objective requires that steps to improve training domain performance should also improve testing domain performance. This meta-learning procedure trains models with good generalization ability to novel domains. 
\citet{balaji2018metaDG}  The objective of domain generalization is explicitly modeled by learning a regularizer that makes the model trained on one domain to perform well on another domain. 
  We pose the problem of finding such a regularization function in a Learning to Learn (or) meta-learning framework. 
 Experimental validations on computer vision and natural language datasets indicate that our method can learn regularizers that achieve good cross-domain generalization.
\citet{qiao2020metaDG} We are concerned with a worst-case scenario in model generalization, in the sense that a model aims to perform well on many unseen domains while there is only one single domain available for training. We propose a new method named adversarial domain augmentation to solve this Out-of-Distribution (OOD) generalization problem. The key idea is to leverage adversarial training to create "fictitious" yet "challenging" populations, from which a model can learn to generalize with theoretical guarantees. To facilitate fast and desirable domain augmentation, we cast the model training in a meta-learning scheme and use a Wasserstein Auto-Encoder (WAE) to relax the widely used worst-case constraint. 
\citet{verma2020metaDG} Learning to classify unseen class samples at test time is popularly referred to as zero-shot learning (ZSL). If test samples can be from training (seen) as well as unseen classes, it is a more challenging problem due to the existence of strong bias towards seen classes. This problem is generally known as \emph{generalized} zero-shot learning (GZSL). Thanks to the recent advances in generative models such as VAEs and GANs, sample synthesis based approaches have gained considerable attention for solving this problem. These approaches are able to handle the problem of class bias by synthesizing unseen class samples. However, these ZSL/GZSL models suffer due to the following key limitations: (i) Their training stage learns a class-conditioned generator using only \emph{seen} class data and the training stage does not \emph{explicitly} learn to generate the unseen class samples; (ii) They do not learn a generic optimal parameter which can easily generalize for both seen and unseen class generation; and (iii) If we only have access to a very few samples per seen class, these models tend to perform poorly. In this paper, we propose a meta-learning based generative model that naturally handles these limitations. The proposed model is based on integrating model-agnostic meta learning with a Wasserstein GAN (WGAN) to handle (i) and (iii), and uses a novel task distribution to handle (ii). 
\citep{li2021metaDG} Zero-shot learning (ZSL) aims to transfer knowledge from seen classes to semantically related unseen classes, which are absent during training. The promising strategies for ZSL are to synthesize visual features of unseen classes conditioned on semantic side information and to incorporate meta-learning to eliminate the model's inherent bias towards seen classes. While existing meta generative approaches pursue a common model shared across task distributions, we aim to construct a generative network adaptive to task characteristics. To this end, we propose an Attribute-Modulated generAtive meta-model for Zero-shot learning (AMAZ). Our model consists of an attribute-aware modulation network, an attribute-augmented generative network, and an attribute-weighted classifier. Given unseen classes, the modulation network adaptively modulates the generator by applying task-specific transformations so that the generative network can adapt to highly diverse tasks. The weighted classifier utilizes the data quality to enhance the training procedure, further improving the model performance. Our empirical evaluations on four widely-used benchmarks show that AMAZ outperforms state-of-the-art methods by 3.8\% and 3.1\% in ZSL and generalized ZSL settings, respectively, demonstrating the superiority of our method. Our experiments on a zero-shot image retrieval task show AMAZ's ability to synthesize instances that portray real visual characteristics.
\end{comment}


Meta learning can improve domain generalization in the following ways.
We have a set of domains as training data.
To simulate the domain generalization scenario, a set of training tasks are constructed by sampling disjoint source and target domains for each task from the training domain.
The learning goal makes use of the intuition that gradient steps that improve the performance of the source domain should also improve the performance of the target domain, thereby encouraging the model to generalize to the unseen target domain.
The idea is borrowed from~\citet{li2018metaDG}, and they use MAML for generalization in the field of computer vision.
For the semantic parser, the experimental results of the (English) Spider and Chinese Spider datasets show that the meta-learning target significantly improves the performance of the baseline parser~\cite{wang-etal-2021-meta}.

This idea can also be applied to cross-language transfer learning~\citep{li-etal-2020-learn}.
Suppose we have English (EN), French (FR), and German (DE) as training domains and Japanese (JA) as testing domain, that is, {EN, FR, DE}->JA.
For each training task, we use one of the source languages ​​as a pseudo-target language in turn and use the rest as pseudo-source languages.
Therefore, we hope that meta-learning can borrow knowledge from the source CLT pair: {FR, DE}->EN, {EN, DE}->FR, {EN, FR}->DE to improve the transfer efficiency of the actual target, that is, {EN, FR, DE}->JA.

Above, we only focus on the setting that training and testing examples have different distributions in a task. Training and test tasks can also have different distributions, so domain shift at the task level may also affect meta learning. But this is beyond the scope of this section.

%Below are approaches for CV, not NLP
\begin{comment}
\citet{li2018metaDG} We propose a novel {meta-learning} method for domain generalization. Rather than designing a specific model that is robust to domain shift as in most previous DG work, we propose a model agnostic training procedure for DG. Our algorithm simulates train/test domain shift during training by synthesizing virtual testing domains within each mini-batch. The meta-optimization objective requires that steps to improve training domain performance should also improve testing domain performance. This meta-learning procedure trains models with good generalization ability to novel domains. 
\citet{balaji2018metaDG}  The objective of domain generalization is explicitly modeled by learning a regularizer that makes the model trained on one domain to perform well on another domain. 
  We pose the problem of finding such a regularization function in a Learning to Learn (or) meta-learning framework. 
 Experimental validations on computer vision and natural language datasets indicate that our method can learn regularizers that achieve good cross-domain generalization.
\citet{qiao2020metaDG} We are concerned with a worst-case scenario in model generalization, in the sense that a model aims to perform well on many unseen domains while there is only one single domain available for training. We propose a new method named adversarial domain augmentation to solve this Out-of-Distribution (OOD) generalization problem. The key idea is to leverage adversarial training to create "fictitious" yet "challenging" populations, from which a model can learn to generalize with theoretical guarantees. To facilitate fast and desirable domain augmentation, we cast the model training in a meta-learning scheme and use a Wasserstein Auto-Encoder (WAE) to relax the widely used worst-case constraint. 
\citet{verma2020metaDG} Learning to classify unseen class samples at test time is popularly referred to as zero-shot learning (ZSL). If test samples can be from training (seen) as well as unseen classes, it is a more challenging problem due to the existence of strong bias towards seen classes. This problem is generally known as \emph{generalized} zero-shot learning (GZSL). Thanks to the recent advances in generative models such as VAEs and GANs, sample synthesis based approaches have gained considerable attention for solving this problem. These approaches are able to handle the problem of class bias by synthesizing unseen class samples. However, these ZSL/GZSL models suffer due to the following key limitations: (i) Their training stage learns a class-conditioned generator using only \emph{seen} class data and the training stage does not \emph{explicitly} learn to generate the unseen class samples; (ii) They do not learn a generic optimal parameter which can easily generalize for both seen and unseen class generation; and (iii) If we only have access to a very few samples per seen class, these models tend to perform poorly. In this paper, we propose a meta-learning based generative model that naturally handles these limitations. The proposed model is based on integrating model-agnostic meta learning with a Wasserstein GAN (WGAN) to handle (i) and (iii), and uses a novel task distribution to handle (ii). 
\citep{li2021metaDG} Zero-shot learning (ZSL) aims to transfer knowledge from seen classes to semantically related unseen classes, which are absent during training. The promising strategies for ZSL are to synthesize visual features of unseen classes conditioned on semantic side information and to incorporate meta-learning to eliminate the model's inherent bias towards seen classes. While existing meta generative approaches pursue a common model shared across task distributions, we aim to construct a generative network adaptive to task characteristics. To this end, we propose an Attribute-Modulated generAtive meta-model for Zero-shot learning (AMAZ). Our model consists of an attribute-aware modulation network, an attribute-augmented generative network, and an attribute-weighted classifier. Given unseen classes, the modulation network adaptively modulates the generator by applying task-specific transformations so that the generative network can adapt to highly diverse tasks. The weighted classifier utilizes the data quality to enhance the training procedure, further improving the model performance. Our empirical evaluations on four widely-used benchmarks show that AMAZ outperforms state-of-the-art methods by 3.8\% and 3.1\% in ZSL and generalized ZSL settings, respectively, demonstrating the superiority of our method. Our experiments on a zero-shot image retrieval task show AMAZ's ability to synthesize instances that portray real visual characteristics.
\end{comment}


Domain generalization is also an important research topic of NLP.
Recently, pre-training large-scale LM and fine-tuning downstream labeled data is one way to improve domain generalization.
For example, by pre-training a multilingual LM on multilingual data, a model fine-tunes by one language's labeled data can be extended to multiple languages.
Multilingual pre-training language model methods usually involve two problems~\citep{li-etal-2020-learn}: (1) simply fine-tuning may not adapt general-purpose multilingual representations to be task-aware on low-resource languages; (2) ignore how cross-lingual adaptation happens for downstream tasks. 
On the other hand, the existing pre-training model adaptation method does not consider the result on new domains after fine-tuning.

\subsection{Meta-learning with a monolithic dataset}  %(Daniel)
\label{sec:task-generation}

%Beyond using relevant corpora but differing in certain attributes such as domains, languages, or tasks, 
\textit{Meta-training tasks} $\mathcal{T}_{train}$ can be constructed with one monolithic dataset (\citet{li2020learning, pasunuru2020fenas, wang2020hat, jiang2019improved, maclaughlin2020evaluating, Wu:EMNLP19, Chien:INTERSPEECH19, learningToLearn:metaNLP21}).
First, the training set of one dataset $D$ is split into support partition, $S_p$, and query partition, $Q_p$. Two subsets of examples are sampled from $S_p$ and $Q_p$ as the support set, $S$, and query set, $Q$, respectively. 
In each episode, model parameters $\theta$ are updated with $S$, and then the losses are computed with the updated model and $Q$.
The meta-parameters $\phi$ are then updated based on the losses, as the meta-learning framework introduced in Section~\ref{sec:background}.  
The test set of $D$ is used to build $\mathcal{T}_{test}$ for evaluation.
The setting is commonly adopted in NAS research. 
As compared to constructing $\mathcal{T}_{train}$ from multiple relevant corpora, which are often not available, building $\mathcal{T}_{train}$ with one dataset makes meta-learning methodology more applicable. 
%developing and evaluating ML techniques is still the dominating benchmarking scenario, 
Besides, results obtained from one dataset are more comparable with existing NLP studies. 
However, only using single data stream makes the resulting models less generalizable to various attributes such as domains and languages.  

\subsection{Task Augmentation} % (Thang) % Thang Vu: combine other and task augmentation? revisit later
Task augmentation
Task augmentation approaches in meta-learning can be categorized in two main directions: a) augmenting tasks means spliting training data from one single task in homogenous partitions that allows applying meta learning techniques and therefore improve the performance and b) augmenting tasks is similarly understood as data augmentation in supervised learning methods. In meta-learning, data augmentation becomes task augmentation because the training data in meta learning is a collection of tasks. To do so, NLP specific methods have been proposed in both categories.

In the first category, the main question is to determine which data points should belong to the same data partition. ...
In the second category, the main question is how to be able to construct a massive amount of tasks in an effient way. ... 


%Suppose we use a learning-to-init approach to learn a set of initialization parameters from two-class classification tasks. In that case, the parameters cannot be used to initialize three-class classification tasks. 
%Consider the problmes are different classification tasks, and different classification tasks have different numbers of classes.In such case, there is no intuitive way to use a unified network architecture to deal with all the classification tasks. In classification tasks, each class has a class-specific head.

%\item ProtoMAML \citep{van-der-heijden-etal-2021-multilingual} -> This is for multilingual 

%They use the following datasets: (1) entity typing: CoNLL-2003 (Sang and De Meulder, 2003), MIT-Restaurant (Liu et al., 2013); (2) rating classification: we use the review ratings for each domain from the Amazon Reviews dataset (Blitzer et al., 2007) and consider a 3-way classification based on the ratings; (3) text classification: social-media datasets from crowdflower4. For sentiment classification we use 4 domains of Amazon reviews (Blitzer et al., 2007) and for NLI we use a scientific entailment dataset (SciTail) (Khot et al., 2018).

%as shown in Section~\ref{sec:cross-problem}. %We will also survey the trend of generating tasks from a single corpus in Section~\ref{sec:task-generation}.
%(e.g., two English datasets on DST tasks in travel or restaurant domains, three MT corpora translating the same English sentence to Germany, French, or Japanese).  

\begin{table*}[ht]
\label{tab:learn-to-init}
  \centering
  \small
  \caption{Summary of learn-to-init variants. 
This paper contains the following information. 
  (1) Approach: There are many variants in the learn-to-init family.
  The
  Typical MAML has large computation intensity, so the first-order approximation (MAML, Reptile) is widely used. 
  %How about NLP applications? In NLP applications, can we use the original favor? Or approximation is needed? 
  (2) How to Initialize the Initialization: Learn-to-init approaches aim at learning the inital parameters. 
  But where does the initialization of MAML comes from? 
  We found that using self-supervised pre-training as initialization is common. 
  %One can use self-supervised pre-training as initialization, one can use multi-task learning for initialization, one can use self-supervised learning and then multi-task learning as initialization. 
  (3) Fine-tuning the whole model is not needed. ANIL fine-tunes the last layer, BOIL fine-tunes the layers, except the last layers. In NLP, which layers are suitable to be fine-tuned. Is it application-dependent? }
  \label{table:methods}
  \begin{tabular}{l|l|l|l|l|l|l|}
    \toprule
Work & Conference & Year & Approach & How to Initailize the Initailization & What to fine-tune & note \\
    \midrule
\citep{Bansal:arXiv19}&COLING & 2020 & MAML & pretrain, BERT & whole( w/ per-layer learning rate) & \\
\citep{Li_Wang_Yu_2020}&AAAI & 2020 & MAML & no & whole & \\
\citep{unsupervisedMT-acl21}&ACL & 2021 & MAML & pretrain, XLM & whole &  \\ 
\citep{Gu:EMNLP18}&EMNLP & 2018 & FOMAML & pretrain embedding w/ FastText & whole / emb+enc / emb (emb+enc is the best) & using universal multilingual representation, embedding is inited by  fasttext \\
\citep{multiparsing}&arXiv & 2021 & FOMAML & mBERT + pre-train on English & whole & \\
\citep{chen-etal-2020-low}&EMNLP & 2020 & Reptile & pretrain, BART & whole & \\
\citep{Huang:ACL20}&ACL & 2020 & MAML & BERT & BERT is fixed (only for embedding) & \\
\citep{wang-etal-2021-variance}&NAACL & 2021 & FOMAML & only use Glove embedding & whole & apply on several tasks \\
\citep{dingliwal-etal-2021-shot}&EACL & 2021 & REPTILE & Roberta-Large & whole & finetune multiple times for mean \& STD \\
\citep{Qian:ACL19}&ACL & 2019 & MAML & pretrained Glove embedding & whole & \\
\citep{ST-dialogue-AAAI21}&AAAI & 2021 & MAML & pretrained Glove embedding & whole & \\
\citep{Madotto:ACL19}&ACL & 2019 & MAML & pretrained Glove embedding & whole & \\
\citep{dai-etal-2020-learning}&ACL & 2020 & MAML & no & whole & \\
\citep{Hsu:ICASSP20}&ICASSP & 2020 & FOMAML & pretrain, Multilingual ASR & whole & \\
\citep{ASR-sample-AAAI21}&AAAI & 2021 & MAML & not mentioned & whole & \\ 
\citep{Winata:INTERSPEECH2020}&Interspeech & 2020 & MAML & pretrain, Librispeech & whole & \\
\citep{Klejch:ASRU19}&ASRU & 2019 & FOMAML & no & whole & The last paragraph of Section 2.3 mentioned first order \\
\citep{SPmetaNLP21}&metaNLP ACL & 2021 & MAML, FOMAML & no & whole & FOMAML is better for without noise; MAML is better for with noise \\
\citep{Indurthi:arXiv19}&ICASSP & 2020 & MAML & no & whole & \\
\citep{Winata:ACL2020}&ACL & 2020 & MAML & no & whole & \\
\citep{SP-ICASSP21}&ICASSP & 2021 & MAML, ANIL & pretrain 50, 84 epochs & MAML whole, ANIL(encoder+decoder, or separator) & MAML is the best in most cases, but ANIL_s is better for libri+noise \\
\citep{ke-etal-2021-pre}&NAACL & 2021 & MAML & pretrain,  Chinese BERT-Base&whole & special application \\
\citep{xia-etal-2021-metaxl}&NAACL & 2021 & meta-learning based, called MetaXL in the paper & pretrain, mBERT and XLM-R&whole&NER / sentiment \\
%\citep{}%EMNLP & 2020 & ? & pretrain, BERT & whole & not MAML-based \\
\citep{Dou:EMNLP19}&EMNLP & 2019 & MAML,First-Order MAML,Reptile&pretrain, BERT & whole & \\
\citep{Obamuyide:ACL19}&ACL & 2019 & First-Order MAML & No & whole & \\
\citep{Lv:EMNLP19}&EMNLP & 2019 & MAML & & whole & using reinforce agent \\
%\citep{}%EMNLP & 2019 & ? & yes, pretained entity embedding & no fine-tune & not MAML-based \\
\citep{holla-etal-2020-learning}&EMNLP-findings & 2020 & Proto, FOMAML, FOMAML+Proto & pretrained Glove embedding, ELMo, BERT & only BERT in finteuned & \\
\citep{huang-etal-2020-towards-low}&EMNLP-findings & 2020 & MAML & no & whole & \\
%\citep{}%AAAI & 2020 & unknown! & no & whole & ?????? \\
\citep{Mi:IJCAI19}&IJCAI & 2019 & MAML & no & whole & It looks like the whole model is fined-tuned, but unclear in the paper \\ 
\citep{wang-etal-2021-meta}&NAACL & 2021 & DG-MAML & BERT & whole & MAML's variant, minimize support set and query set loss at the same time ... \\
\citep{ranking-acl21}&ACL-IJCNLP & 2021 & Meta-reweight (describe in comment) & BERT for ranking, T5 for generating data&whole (both BERT and T5, but T5 is not meta-learned) & \\ %先meta learn不同筆data的weight (用類似MAML的bilevel optimization，inner update model，outer update weight)，再用學到的weight走一步正常的traiining
\citep{conklin2021meta}&ACL & 2021 & DG-MAML & no & whole & \\
\citep{mhamdi-etal-2021-x}&NAACL & 2021 & MAML & BERT pretrained on train split of English & whole & \\ %分成meta train和meta adapt，meta train的support set是high-resource language，meta train的query和meta adapt的support&query都是low-resource
\citep{nooralahzadeh-etal-2020-zero}&EMNLP & 2020 & MAML & ESIM(LSTM) for MNLI, En-BERT and Multi-BERT for XNLI, XLM and XLM-RoBERTa for QA & whole & selecting on or two auxilary langauges for MAML \\ 
\citep{MetaKD-arXiv21}&ECAI & 2020 & MAML & teacher yes, student no (so no ?) & whole & \\ %有兩個student，s1透過quiz examples update teacher to T', then T' distils to s2 %(European Conference on Artificial Intelligence)
%\citep{}&arXiv & 2020 & MAML(parameters are updated per batch-of-tasks instead of per task) & yes & whole & is this paper related to HLP? No HLP experiments \\
\citep{garcia-etal-2021-cross}&Adapt-NLP & 2021 & MAML & yes & whole & the meta-tasks is structure to a tree (relatedness between tasks), to MAML gradient propogates according to that tree \\
\citep{van-der-heijden-etal-2021-multilingual}&EACL & 2021 & FOMAML+proto & XLM-RoBERTa & & \\
\citep{bansal-etal-2020-self}&EMNLP & 2020 & optimization-based meta-learning (OBML?) & pretrain, BERT & whole & This work uses self-supervised tasks in meta-learning, instead of supervised tasks \\
\citep{murty-etal-2021-dreca}&NAACL & 2021 & FOMAML & pretrain, BERT & whole & \\
\citep{hua-etal-2020-shot}&EMNLP & 2020 & Reptile & No & Whole & \\     
     
     \hline
    \bottomrule
  \end{tabular}
\end{table*}
%preliminary results for survey: https://docs.google.com/spreadsheets/d/1oOjwWLWqmvhWizE3lugQWEUpUKggyni9u6nOGy_ratg/edit?usp=sharing 

==> previous.tex <==
\section{Note for Learning to Initialize (recent conference)}

\subsection{Applications}

multiple acpplications?
Learning to Few-Shot Learn Across Diverse Natural Language Classification Tasks

Hypernymy Detection for Low-Resource Languages via Meta Learning, ACL 2020
https://slideslive.com/38929011/hypernymy-detection-for-lowresource-languages-via-meta-learning

Metaner: Named entity recognition with meta-learning?

MEtaMT, a meta learning method leveraging multiple domain
data for low resource machine translation., AAAI

Meta-Learning with Sparse Experience Replay for Lifelong Language Learning
Nithin Holla, Pushkar Mishra, Helen Yannakoudakis, Ekaterina Shutova

KEML: A Knowledge-Enriched Meta-Learning Framework for Lexical Relation Classification (not MAMT?)
Chengyu Wang, Minghui Qiu, Jun Huang, Xiaofeng He

\subsubsection{Parsing}

Low-Resource Domain Adaptation for Compositional Task-Oriented Semantic Parsing
Xilun Chen, Asish Ghoshal, Yashar Mehdad, Luke Zettlemoyer, Sonal Gupta

\subsubsection{DST}
Can I consider DST as one kind of parsing?

Meta-Reinforced Multi-Domain State Generator for Dialogue Systems
dialogue state tracking (DST)~\cite{Huang:ACL20}. 
http://slideslive.com/38929369
I think this one can be considered as typical MAML.
RL is another story.

Towards Low-Resource Semi-Supervised Dialogue Generation with Meta-Learning, EMNLP 2020 finding 
This is also dialogue state tracking
This one use unlabeled data, which is novel.
I think this one follows the above paper.
But I cannot understand this one. 
It is wierd. 

% First-order metalearning is a widely-used method in practice. %Lee: is the approach only for FOMAML?
\citep{wang-etal-2021-variance}
MAML struggles to learn on diverse task distributions (all papers cited in the paper are not NLP).
 It has been observed in many previous works (all papers cited here are federated learning) that local update methods, including first-order meta-learning, performing multiple optimization steps on local data can lead to overfitting to atypical local data. 
 In the context of first-order meta-learning, due to the large variance of the gradient estimator, task adaptation will drive task-specific models to move away from each other, resulting in that the gradients used
in meta update have diverse directions. Furthermore, since the difference in gradient magnitudes will also be large, the task with a much larger gradient in magnitude will dominate the task adaptation. As a result, the meta update will overfit to this dominating task.
The above gradient variance issue, i.e., the large variance from the gradient estimator, is significant in NLP applications since many NLP datasets have diverse properties, and the tasks for meta-learning in NLP applications also have their unique characteristics.
For example, the MultiWOZ dataset (Budzianowski et al., 2018) for dialog systems and the Spider dataset (Yu et al., 2018) for semantic parsing, both consist of complex and cross domain examples.
The paper proposes to reduce the variance of the gradient estimator used in task adaptation. The core of the algorithm is to introduce a novel variance reduction term to the gradient estimation when performing the task adaptation.
(This paper only include classification and dailogue state tracking)

%N-Shot Learning for Augmenting Task-Oriented Dialogue State Tracking
%Nancy's paper
%But nothing related to meta 

\subsection{Dialouge}

\subsubsection{End-to-end}
\cite{Qian:ACL19}
Kun Qian and Zhou Yu. 2019. Domain adaptive dialog generation via meta learning. In ACL. 
https://vimeo.com/384728415
I think this one is task oriented.

MALA: Cross-Domain Dialogue Generation with Action Learning, AAAI 2020

A Student-Teacher Architecture for Dialog Domain Adaptation under the Meta-Learning Setting, AAAI 2021
Numerous new dialog domains are being created every day while collecting data for these domains is extremely costly since it involves human interactions. Therefore, it is essential to develop algorithms that can adapt to different domains efficiently when building data-driven dialog models. The most recent researches on domain adaption focus on giving the model a better initialization, rather than optimizing the adaptation process. We propose an efficient domain adaptive task-oriented dialog system model, which incorporates a meta-teacher model to emphasize the different impacts between generated tokens with respect to the context. We first train our base dialog model and meta-teacher model adversarially in a meta-learning setting on rich-resource domains. The meta-teacher learns to quantify the importance of tokens under different contexts across different domains. During adaptation, the meta-teacher guides the dialog model to focus on important tokens in order to achieve better adaptation efficiency. We evaluate our model on two multi-domain datasets, MultiWOZ and Google Schema-Guided Dialogue, and achieve state-of-the-art performance.

I think this is not based on MAML.
Learning to customize model structures for few-shot dialogue generation tasks, ACL 2020 ***

\subsubsection{Chatbot}

Meta NLG
Meta-Learning for Low-resource Natural Language Generation in Task-oriented Dialogue Systems
\cite{Mi:IJCAI19}
This one also has good citation.

\cite{Madotto:ACL19}
Personalizing Dialogue Agents via Meta-Learning
Collecting many dialogs involving a specific persona is expensive, while it is challenging to capture a persona using only a few conversations. Thus, meta-learning comes into play for learning persona with few-shot example conversations~\cite{Madotto:ACL19}.

\subsubsection{Relation Classification}

\cite{Obamuyide:ACL19}
%Abiola Obamuyide and Andreas Vlachos. 2019. Modelagnostic meta-learning for relation classification with limited supervision. In ACL.
This one is naive version of MAML for relation classificaiton.

\cite{Bose:arXiv19}
This paper is meta-graph. It is not accepted by any conference, and it is weird in my view point.

Adapting Meta Knowledge Graph Information for Multi-Hop Reasoning over Few-Shot Relations
\cite{Lv:EMNLP19} (Has a figure of relation freq.)

Tackling Long-Tailed Relations and Uncommon Entities in Knowledge Graph Completion
\cite{wang2019tackling} (Has a figure of relation freq.)
This one is not MAML based!

This paper is about speech recognitoin, which takes each langauge as a training task.
Adversarial Meta Sampling for Multilingual Low-Resource Speech Recognition
Yubei Xiao, Ke Gong, Pan Zhou, Guolin Zheng, Xiaodan Liang, Liang Lin
studying how to sample the training tasks during across task training. 
%Dose the below paper use the similar idea
Minimax and Neyman-Pearson Meta-Learning for Outlier Languages (ACL finding) -> different languages have different probabilities to be sampled ???


%Unsupervised Neural Machine Translation for Low-Resource Domains via Meta-Learning
\citep{unsupervisedMT-acl21}
To address this issue, this paper presents a novel meta-learning algorithm for unsupervised neural machine translation (UNMT) that trains the model to adapt to another domain by utilizing only a small amount of training data. We assume that domain-general knowledge is a significant factor in handling data-scarce domains.

%Learning to Learn to Disambiguate: Meta-Learning for Few-Shot Word Sense Disambiguation
%Meta-Learning with Variational Semantic Memory for Word Sense Disambiguation
Semantic memory encapsulates prior experiences seen throughout the lifetime of the model, which aids better generalization in limited data settings. Our model is based on hierarchical variational inference and incorporates an adaptive memory update rule via a hypernetwork. This is based on proto.



Don’t Miss the Labels: Label-semantic Augmented Meta-Learner for Few-Shot Text Classification, ACL 2021 finding, (cannot find arxiv link)

Meta-Learning Adversarial Domain Adaptation Network for Few-Shot Text Classification, ACL 2021 (cannot find arxiv link)

Adaptive Knowledge-Enhanced Bayesian Meta-Learning for Few-shot Event Detection, ACL 2021 finding  
This is metric based

\section{Meta for Domain Adaptation}
There are two aspects. One is Meta learning can be used to solve the problem of domain adaptation.
The another is that meta learning also face the issue of domain mismatch iself, for example, "Two Sides of Meta-Learning Evaluation: In vs. Out of Distribution"

\subsection{General idea}

\subsubsection{Domain adaptation}
%MetaAlign: Coordinating Domain Alignment and Classification for Unsupervised Domain Adaptation
MetaAlign encourages both tasks to be optimized in a coordinated way, which maximizes the inner product of the gradients of the two tasks during training.
The basic idea is that to learn a classidier that is good at alignemnt.
It looks like the classification is the in-task training.
The alignment is the in-tast testing.
(This paper has a pretty figure.)

\subsubsection{Domain generatlization}
%Learning to Generalize: Meta-Learning for Domain Generalization, AAAI 2018 
% This one is weird. I cannot really understand.

%Episodic Training for Domain Generalization

%MetaReg: Towards Domain Generalization using Meta-Regularization

%Learning to Learn Single Domain Generalization
Using one domain data to generate mutiple domains. Then use meta learning. 

%Domain Generalization via Model-Agnostic Learning of Semantic Features %%%
The paper seems clear (I do not read it) 
Below is from the paper:
The episodic training paradigm, originated from model-agnostic meta-learning (MAML) [10], has been introduced to address domain generalization [1, 26, 27, 31].
Epi-FCR [27] alternates domain-specific feature extractors and classifiers across domains via episodic training, but without using inner gradient descent update. 
The method of MLDG [26] closely follows the update rule of MAML, back-propagating the gradients from an ordinary task loss on meta-test data. A limitation is that using the task objective might be sub-optimal, as it is highly abstractedfrom the feature representations (only using class probabilities). Moreover, it may not well fit the scenario where target data are unavailable (as pointed out by Balaji et al. [1]). 
A recent method, MetaReg [1], learns a regularization function (e.g., weighted L1 loss) particularly for the network’s classification layer, excluding the feature extractor. 
Li et al. [31] propose a feature-critic network which learns an auxiliary meta loss (producing a non-negative scalar) depending on output of the feature extractor. 
Both [1] and [31] lack notable guidance from semantics of feature space, which may contain crucial domain-independent ‘general knowledge’ for model generalization. 
The proposed method is orthogonal to previous work, proposing to enforce semantic features via global class alignment and local sample clustering, with losses explicitly derived in an episodic learning procedure.

%MetaNorm: Learning to Normalize Few-Shot Batches Across Domains %ICRL２０２１
This paper proposes an lightweight method for cross-domain few-shot learning, using a meta-learning approach to predict batch normalization statistics.

\subsubsection{Zero shot?}
%Meta-Learning for Generalized Zero-Shot Learning
In each task, the training and testing are disjointed. 
This paper learning to synthesize examples from unseen classes,

\subsection{NLP applications}

%Meta-Learning for Domain Generalization in Semantic Parsing %%%
\citep{wang-etal-2021-meta} %This paper has an brief overview about Meta-Learning for NLP (but I do not check it.) 
This paper aims at Zero-shot semantic parsing. At training time, a parser observes instances for the database concert singer. At test time, it needs to generate SQL for questions pertaining to the unseen database farm.
We apply a modelagnostic training algorithm that simulates zeroshot parsing by constructing virtual train and test sets from disjoint domains. The learning objective capitalizes on the intuition that gradient steps that improve source-domain performance should also improve target-domain performance, thus encouraging a parser to generalize to unseen target domains. Experimental results on the (English) Spider and Chinese Spider datasets show that the meta-learning objective significantly boosts the performance of a baseline parser.

%Few-Shot Text Ranking with Meta Adapted Synthetic Weak Supervision
\citep{ranking-acl21}
This paper is about domain adaptation for ranking in IR. It looks like meta leanring is used for sample weighing. %But I do not truly understand this one

Meta-Learning to Compositionally Generalize, ACL 2021

\subsubsection{cross-lingual}
Here in a training task, the training examples are from one langauge, while the testing examples are from the other.


%X-METRA-ADA: Cross-lingual Meta-Transfer learning Adaptation to Natural Language Understanding and Question Answering
\citep{mhamdi-etal-2021-x}
The meta-train stage transfers from the source to the target languages, while the meta-adaptation further adapts the model to the target language. The application is few-shot if the test language is seen in any stage of X-METRA-ADA; or zeroshot if the test language is unseen.

%Zero-Shot Cross-Lingual Transfer with Meta Learning %XMAML
\citep{nooralahzadeh-etal-2020-zero}
This introduce a cross-lingual meta-learning framework (XMAML). 
There is a follow-up paper in our workshop. (I believe there are two.)

%Learn to Cross-lingual Transfer with Meta Graph Learning Across Heterogeneous Languages
\citep{li-etal-2020-learn} %-> This one is metric based.
MGL can learn to cross-lingual transfer by extracting meta-knowledge from historical CLT experiences (tasks), making mPLM insensitive to low-resource languages.

Meta-learning for fast cross-lingual adaptation in dependency parsing

Attribute-Modulated Generative Meta Learning for Zero-Shot Classification %not NLP

Cross-Lingual Transfer with MAML on Trees, EACL

Multilingual and cross-lingual document classification: A meta-learning approach

\subsection{Meta KD}
This is learn to teach!

%Meta Learning for Knowledge Distillation
\citep{metakd-meta} This one is based on MAML. (BERT is used)

%Meta-KD: A Meta Knowledge Distillation Framework for Language Model Compression across Domains
\citep{metakd-acl21} This is proto based ... I do not truly understand this one. 
Pan et al. (2020) proposed a framework to train a meta-teacher across domains that can better fit new domains with meta-learning. Then, traditional KD is performed to transfer the knowledge from the meta-teacher to the student. (description from other papers)

%Benlin Liu, Yongming Rao, Jiwen Lu, Jie Zhou, and Cho-Jui Hsieh. Metadistiller: Network selfboosting via meta-learned top-down distillation. In ECCV, 2020.

%Meta Pseudo Labels. This is a learn to teach paper at CVPR 2021. (This pape has high citation, but I do not have time to go through the papers cite this one.)

%\subsection{Data Selection / Label Correction - integrated into main text}

%Learning to Learn from Noisy Labeled Data, 2018
% Here is an old paper about noisy labeld data with MAML.
% I have never read this one.

%Meta Label Correction for Noisy Label Learning
% \citep{label-correction-aaai21}
% This is a more general meta learning for label correction framework. It did apply this method on BERT-based text classification.

%Balancing training for multilingual neural machine translation.
%\citep{wang2020balancing}
%Differentiable Data Selection can be considered as meta? %This is ACL 2020 paper.

%On Negative Interference in Multilingual Models: Findings and A Meta-Learning Treatment
%\citep{wang-etal-2020-negative}
%The paper presents a meta-learning algorithm that obtains better cross-lingual transferability and alleviates negative interference, by adding language-specific layers as meta-parameters and training them in a manner that explicitly improves shared layers’ generalization on all languages. 

%META BACK-TRANSLATION -> This is ILCR 2021 paper. (But I have never read it ...)


\subsection{Task Augmentation}
%I believe some people have done task augmentation before .
% for example, labeling switching in meta learning without memortization 

%Meta Learning requires Meta Augmentation, NIPS

%Unsupervised learning via meta-learning. ICLR
Hsu et al. (2019) propose CACTUs, a clustering-based approach for unsupervised meta-learning in the context of few-shot label adaptation for images.

%SMLMT
%Self-supervised meta-learning for few-shot natural language classification tasks. EMNLP 2020
\cite{bansal-etal-2020-self}
 Standard meta-learning techniques require many training tasks in order to generalize; unfortunately, finding a diverse set of such supervised tasks is usually difficult. This paper proposes a self-supervised approach to generate a large, rich, meta-learning task distribution from unlabeled text. 
SMLMT creates new self-supervised tasks that improve meta-overfitting but this does not directly address the dataset-as-tasks problem we identify.



%DReCa: A General Task Augmentation Strategy for Few-Shot Natural Language Inference
\citep{murty-etal-2021-dreca}
This work can be considered as dividing a task into smaller one. 
%Adaptation is central to many NLP applications since new concepts and words appear often, leading to distribution shifts. People can effortlessly deal with these distribution shifts by learning these new concepts quickly and we would like our models to have similar capabilities.
 An important prerequisite for successful application of meta-learning is a task-distribution from which a large number of tasks can be sampled to train the meta-learner. While meta-learning is very appealing, applications in NLP have thus far proven challenging due to the absence of a well-defined set of tasks that correspond to re-usable skills. This has led to less effective ad hoc alternatives, like treating entire datasets as tasks.
DRECA is a meta data augmentation strategy that takes as input a set of tasks (entire datasets), and then decomposes them to approximately recover some of the latent reasoning categories underlying these datasets, such as various syntactic constructs within a dataset, or semantic categories such as quantifiers and negation.

%Renkun Ni, Micah Goldblum, Amr Sharaf, Kezhi Kong, and Tom Goldstein. Data augmentation for meta-learning. arXiv preprint arXiv:2010.07092, 2020.
%Huaxiu Yao, Longkai Huang, Linjun Zhang, YingWei, Li Tian, James Zou, Junzhou Huang, and Zhenhui Li. Improving generalization in meta-learning via task augmentation. arXiv preprint arXiv:2007.13040, 2020.
%Meta-Learning with Fewer Tasks through Task Interpolation


%Few-Shot Complex Knowledge Base Question Answering via Meta Reinforcement Learning
\citep{hua-etal-2020-shot}
This paper proposes a meta-reinforcement learning approach to program induction in CQA to tackle the potential distributional bias in questions. Our method quickly and effectively adapts the meta-learned programmer to new questions based on the most similar questions retrieved from the training data. 
Related work: 
Huang et al. (2018) use MAML to learn a Seq2Seq model to convert questions in WikiSQL into SQL queries. %This is the one I know. 
Guo et al. (2019) propose Sequence-to-Action (S2A) by using MAML to solve CQA problems. %Coupling retrieval and meta-learning for contextdependent semantic parsing. % in the table 
They label all the examples in training set with pseudo-gold annotations, then train an encoder-decoder model to retrieve relevant samples and a Seq2Seq based semantic parser to generate actions based on the annotations. Unlike S2A, we introduce a Meta-RL approach, which uses RL to train an NPI model without annotating questions in advance. (NPI: neural program induction. What is that?)



\subsection{Meta + Pre-training}
This may not worths a subsection.
What we have to describe is the difference between self-supervised learning and lnearing to initialize. 

%Pre-training with Meta Learning for Chinese Word Segmentation
\citep{ke-etal-2021-pre}
The objective of most PTMs is to maximize its performance on pretraining tasks, which would lead to the discrepancy between pre-trained models and downstream tasks. The main objective of meta learning is to maximize generalization performance on potential downstream tasks, which prevents pre-trained models from overfitting on pre-training tasks. The meta learning algorithm treats pre-training task as one of the downstream tasks.
Since the discrepancy between pre-training tasks and downstream tasks also exists in other NLP tasks and other languages, the method could be applied to other tasks and languages apart from Chinese word segmentation.

%Meta Fine-Tuning Neural Language Models for Multi-Domain Text Mining
\citep{wang-etal-2020-meta}
This paper proposes an effective learning procedure named Meta Fine-Tuning (MFT), serving as a meta-learner to solve a group of similar NLP tasks for neural language models. Instead of simply multi-task training over all the datasets, MFT only learns from typical instances of various domains to acquire highly transferable knowledge. It further encourages the language model to encode domaininvariant representations by optimizing a series of novel domain corruption loss functions. After MFT, the model can be fine-tuned for each domain with better parameter initialization and higher generalization ability. (I cannot get the core idea of this paepr.)


%MetaXL: Meta Representation Transformation for Low-resource Cross-lingual Learning
\citep{xia-etal-2021-metaxl}
For extremely low-resource languages without large-scale monolingual corpora for pre-training or sufficient annotated data for fine-tuning, transfer learning remains an under-studied and challenging task MetaXL pushes the source (EN) and target (TEL) representations closer to realize a more effective transfer.
It is similar to pre-train a model that can insert adapter (am I right?).

\subsection{meta for lifelong learning (not forgeting)}

There are also two types of meta plus life-long.
Perhaps the two types can be merged. 

\subsubsection{Life-long learning for Meta learning }

Meta learning also suffers from the issue of catestrophic forgeting.
Hence, we have to apply the idea of life-long learning to meta learning.
There are different ways to deal with Meta-Learning in an online framework: the so-called Online-Within-Batch (OWB) framework, where the tasks are processed online but the data within each task are processed in one batch, see [1, 12, 13, 16, 8, 3, 21], or the so-called Online-Within-Online (OWO) framework, where data are processed sequentially both within and across the tasks.
(The above sentence is copied from the paper "Online-Within-Online Meta-Learning" -> I am not able to understand this paper) %%%

%Online Meta-Learning
This is probably the original one. It contains both Life-long learning for Meta learning and Meta learning for Life-long learning. I have read this one.

%Addressing Catastrophic Forgetting in Few-Shot Problems ??? %ICML %%%
This paper focuses on imporving Online Meta-Learning:
Explicitly keeping a memory on previous
data often triggers an important question: how should
the carried-forward data be processed in future rounds, in
order to accumulate knowledge? Finn et al. (2019) update
the meta-parameters at each iteration using data sampled
from the accumulated task buffer. This defeats the purpose
of online learning, which by definition means to update the
parameters each round using only the new data encountered.

%Continuous Meta-Learning without Tasks %%% NIPS, 2020

\subsubsection{Meta learning for Life-long learning}

Using meta learning to prevent forgeting.

%Editable neural networks -> This can be considered as fast adaptation? %%% ICLR 2020
 how one can efficiently patch a mistake of the model on a particular sample, without influencing the model behavior on other samples
 It has been used on MT, which is an NLP task. 
 
%Editing Factual Knowledge in Language Models %This one is NLP related %%%


% Efficient Meta Lifelong-Learning with Limited Memory %%%
\citep{wang-etal-2020-efficient}
This paper proposes a meta-lifelong framework. 
This paper changes the training goal of generic representation from how to perform better on the current task to how to adapt to episodic memory efficiently.
This paper focuses on storing limited training examples in memory. -> I believe this is learned by meta???

%Task Agnostic Continual Learning via Meta Learning %%%
shift the focus from less forgetting to faster remembering: to rapidly recall a previously learned task, given the right context as a cue.

%Meta-learnt priors slow down catastrophic forgetting in neural networks %%%

%Continual Quality Estimation with Online Bayesian Meta-Learning, ACL 2021 (cannot find arxiv link)

\section{Note for Other meta learning approaches}
\subsection{Neural network search (NAS)}
Note that most NAS approaches discussed in this section are trained by sampling (sub)tasks from one dataset, and the training/test dataset is usually matched (default setting if not specified in this section). This is different from other meta-learning approaches introduced in this paper, where multiple datasets/languages are usually used, and training and inference conditions are usually mistmatched. 

%Learning Architectures from an Extended Search Space for Language Modeling

\citep{li2020learning} extends the search space of NAS to cover more RNN architectures to increase the expressibility of searched networks. Specifically the work represents the search space as a directed acyclic graph (DAG) containing intra- and inter-cell connection of neurons, and learns the architecture optimization with differentiable architecture search (DARTS). The searched architecture achieves similar or better language modeling performance than Transformer-XL in WikiText-103 \citep{merity2017revisiting} or PTB \citep{mikolov2010recurrent}. The author also demonstates the transferability of learned networks by showing new SOTA on NER tasks with CoNLL dataset.


%FENAS: Flexible and Expressive Neural Architecture Search
\citep{pasunuru2020fenas} proposes FENAS (Flexible and Expressive Neural Architecture Search) to also explore expanding the search space of ENAS with more functions (e.g., skip-based tanh, ReLU) and atomic-level operations (e.g., addition, subtraction, element-wise multiplication). FENAS employs evolutionary algorithm to search network architecture rather than RL, which is utilized in ENAS. FENAS further allows to leverage well-known human-designed architectures, such as LSTM and GRU, as search initialization and as part of searched components in mutation. These designed cells improve the search efficiency and the accuracy of resulting networks. Experiments show that FENAS yields better perplexity in PTB and higher accuracy in GLUE as compared to ENAS, while FENAS requires 5x to 16x more GPU days due to larger search space.


%HAT: Hardware-Aware Transformers for Efficient Natural Language Processing
\citep{wang2020hat} introduces HAT (Hardware-Aware Transformers) to search Transformers architecture optimized for underlying hardware platforms. In HAT, a weigh-shared SuperTransformer is first trained by iteratively optimizing sub-networks (also denoted as SubTransformers) randomly sampled from the SuperTransformer and aggregating the weights over iterations. The SuperTransformer is designed such that any network in the search space can be represented as a sub-network of the SuperTransformer. Then, a MLP network is learned for each hardware to predict latency from architecture. The network takes a feature vector representing the architecture as input. To obtain the latency of architectures for training, architectures are sampled and inference of SubTransformers of the sampled architectures are run on hardware for measuring the latency. The authors leverage this MLP predictor, instead of running inference with architecture in search to obtain exact latency, to improve search efficiency. After that, evolution search is conducted to optimize network architectures for latency and accuracy, which is estimated with the MLP predictor and the validation loss of SubTransformer using weights inherited from SuperTransformer, respectively. The weight sharing between SuperTransformer and SubTransformer is also for efficiency. Lastly, a network with the optimized architecture is retrained either from scratch or from SubTransformer's weights as the final model. The authors measure the efficacy of HAT with translation tasks on WMT’14 En-De, WMT’14 En-Fr, WMT’19 En-De, and IWSLT’14 De-En datasets and on Raspberry Pi ARM CPU, Intel Xeon CPU, and Nvidia TITAN Xp GPU. Empirically, HAT yields 3x speedup and 3x size reduction compared to Transformer-Big with similar BLEU scores. HAT is also 12000x faster than Evolved transformer baseline that leverage NAS for optimizing architecture.

%Continual and Multi-Task Architecture Search
\citep{pasunuru2019continual} presents  continual architecture search (CAS) by combining Efficient Neural Architecture Search (ENAS) \citep{pham2018efficient} and continual learning. CAS aims to sequentially training of networks on several tasks without forgetting previously learned objective. The authors also propose a multi-task version of architecture search to optimize a unified structure for many tasks. Effectiveness of proposed techniques in sequential continual learning and parallel multi-task training is explored on GLUE.

%Improved differentiable architecture search for language modeling and named entity recognition
\citep{jiang2019improved} improves differentiable NAS by redesigning its search space for natural language processing. The work also pioneers in the application of NAS to NLP tasks other than language modeling. The proposed approach demonstates SOTA or competitive performance in CoNLL-2003 NER data and PTB language modeling respectively.

%Evaluating the Effectiveness of Efficient Neural Architecture Search for Sentence-Pair Tasks
\citep{maclaughlin2020evaluating} explores the application of ENAS \citep{pham2018efficient} to two sentence pair classification tasks, paraphrase detection and semantic textual similarity. Experiments are conducted on three datasets (MRPC \citep{dolan2005automatically}, SICK \citep{marelli2014sick}, STS-B \citep{cer2017semeval}).

%Co-evolution of language and agents in referential games

\citep{dagan2021co} investigates the problem of referential games, where the goal is to build a learning environment for neural agents to learn language and communicate functionally. The authors employ DARTS to simulate a practical characteristic in the environment that the individual agent, the agent cohorts, and the learned language co-evolve. Modeling the co-evolution in environment paves the way to study the problem of language emergence.

%(ASR) Yi-Chen Chen, Jui-Yang Hsu, Cheng-Kuang Lee, and Hungyi Lee. 2020b.  DARTS-ASR: Differentiable architecture search for multilingual speech recognition and adaptation. In INTERSPEECH.
%(ASR) Ahmed Baruwa, Mojeed Abisiga, Ibrahim Gbadegesin, and Afeez Fakunle. 2019. Leveraging end-to-end speech recognition with neural architecture search. In IJSER.
%(Keyword spotting) Hanna  Mazzawi, Xavi  Gonzalvo, Aleks  Kracun,  Prashant Sridhar,  Niranjan Subrahmanya, Ignacio Lopez Moreno, Hyun Jin Park, and Patrick Violette. 2019. Improving key-word spotting and language identification via neural architecture search at scale. In INTERSPEECH.

\subsection{Learning to optimize}
% Soft Layer Selection with Meta-Learning for Zero-Shot Cross-Lingual Transfer
\citep{learningToOptimize:metaNLP21} studies the problem of zero-shot cross-lingual transfer and proposes a meta-optimizer. The meta-optimizer is trained to soft-select portion of parameters in pre-trained networks to be frozen during fine-tuning. The training is also done episodically to simulate the zero-shot transfer scenario. The authors show the proposed meta-optimizer outperforms competitive baselines including XMAML \citep{nooralahzadeh-etal-2020-zero} in the studied problem with a task of Natural Language Inference. % XNLI dataset \citep{conneau2018xnli}

% Jen-Tzung Chien and Wei Xiang Lieow. 2019. Meta learning for hyperparameter optimization in dialogue system. In INTERSPEECH.

\subsection{Learning the learning algorithm}

% Jiawei Wu, Wenhan Xiong, and William Yang Wang. 2019. Learning to learn and predict:  A meta-learning approach for multi-label classification

% Learning to Learn Words from Visual Scenes https://arxiv.org/abs/1911.11237v3 ECCV 2020

% Zero-Shot Compositional Concept Learning
\citep{learningToLearn:metaNLP21} proposes EpiCA (episode-based cross-attention), a framework of learning the cross attention policy over images and texts, to improve the representation of concepts. EpiCA trains a network with an episode-based training strategy to the policy for fusing multi-modal information. The paper demonstrates empirically the efficacy of EpiCA in improving zero-shot compositional concept learning (ZSCL) by achieving new SOTA on two public ZSCL benchmakrs, MIT-States \citep{isola2015discovering} and UT-Zappos \citep{yu2017semantic}.

%\subsection{Learning to data selection - integrated into main text}

% sample reweighting

%Balancing Training for Multilingual Neural Machine Translation
%\citep{wang2020balancing} investigates the common challenge of imbalanced training examples across languages in multilingual machine translation (MT). Conventionally, up-sampling languages with less resources is utilized, and such mechanism is controlled by developer-tuned hyperparameters. The authors propose Differentiable Data Selection (DDS) % there is another paper about DDS earlier than this one, from the same authors. 
%to parameterize the sampling strategies. DDS is trained with episodes and REINFORCE algorithm to optimize parameters of sampling and MT models in an alternating way.
% episodes are built with each source-target language pair and training/evaluation split

%Meta-Learning for Effective Multi-task and Multilingual Modelling
%\citep{tarunesh2021meta} studies knowledge transferring across tasks and languages. The authors combine Reptile and DDS to learn from 6 different languages (en, hi, es, de, fr, and zh) and 5 different tasks (QA, NLI, paraphrase identification, POS tagging, and NER). The proposed approach is trained by episodically iterating through different task-language pairs. The approach demonstrates comparable performance against competitive multi-task learning baselines in both zero-shot and fully supervised settings on XTREME multilingual benchmark dataset \citep{hu2020xtreme}.



\section{Additional useful informaiton}
There are some survey papers:
\begin{itemize}
    \item Meta-learning for Few-shot Natural Language Processing: A Survey
    \item Few-Shot Named Entity Recognition: A Comprehensive Study
    \item Learning from Very Few Samples: A Survey
    \item A survey on recent approaches for natural language processing in low-resource scenarios
\end{itemize}

dataset:
Eleni Triantafillou, Tyler Zhu, Vincent Dumoulin, Pascal Lamblin, Utku Evci, Kelvin Xu, Ross Goroshin, Carles Gelada, Kevin Swersky, Pierre-Antoine Manzagol, and Hugo Larochelle. 2020. Meta-dataset: A dataset of datasets for learning to learn from few examples. In International Conference on Learning Representations.

\section{TODO}

Aug 24 meeting
\begin{enumerate}
    \item Finalize tables architecture (what each row / column stands for), similar to tables in https://arxiv.org/pdf/2107.13586.pdf (ddl next meeting). Candidate to put:
    \begin{enumerate}
        %\item number of meta-training task
        \item application v.s. datasets v.s. learning target v.s. methods v.s. how to construct task
        \item MAML: initialization of MAML
        \item meta learning v.s. xxx learning (life long learning, multi-task learning, domain adaptation ...)
        \item Table for learning to compare
        \item (?) Table for other methods
    \end{enumerate}
    \item 2021 Sep goal: finalize paper architecture, who is responsible for what
    \item 2021 Oct goal:
    \item 2021 Nov goal:
    \item 2021 Dec goal:
    \item 2022 Feb goal: editing (shortening, proofreading, making things consistent), submit to TACL end of 2022 Feb (10 page, no appendix)
\end{enumerate}

Old discussion:
\begin{enumerate}
    \item relation between meta learning and oher technology
    \item benchmarking dataset (everyone)
    \item add new papers to each category (Hung-yi: learning to init, Thang: learning to compare, Daniel: others)
    \item think about the taxonomy (Hung-yi: learning to init, Thang: learning to compare, Daniel: others)
    \item COMMUNICATION: sync in overleaf and more meetings in July (weekly) 
\end{enumerate}






\section{Brief Description}
Deep learning based natural language processing (NLP) has become the mainstream of research in recent years and significantly outperforms conventional methods. However, deep learning models are notorious for being data and computation hungry. 
These downsides limit such models' application from deployment to different domains, languages, countries, or styles, since collecting in-genre data and model training from scratch are costly.
The long-tail nature of human language makes challenges even more significant. 

Meta-learning, or ‘Learning to Learn’, aims to learn better learning algorithms, including better parameter initialization, optimization strategy, network architecture, distance metrics, and beyond. Meta-learning has been shown to allow faster fine-tuning, converge to better performance, and achieve outstanding results for few-shot learning in many applications. 
Meta-learning is one of the most important new techniques in machine learning in recent years. 
There is a related tutorial in ICML 2019\footnote{\url{https://sites.google.com/view/icml19metalearning}} and a related course at Stanford\footnote{\url{http://cs330.stanford.edu/}}, but most of the example applications given in these materials are about image processing. 
It is believed that meta-learning has excellent potential to be applied in NLP, and some works have been proposed with notable achievements in several relevant problems, e.g., relation extraction, machine translation, and dialogue generation and state tracking. 
However, it does not catch the same level of attention as in the image processing community. 

In the tutorial, we will first introduce Meta-learning approaches and the theory behind them, and then review the works of applying this technology to NLP problems. 
Table~\ref{table:ref} summarizes the content this tutorial will cover.
This tutorial intends to facilitate researchers in the NLP community to understand this new technology better and promote more research studies using this new technology.


\section{Type of the tutorial}
The type of tutorial is \textbf{Cutting-edge}. 
Meta-learning is a newly emerging topic. 
The area of natural language processing has seen a growing number of papers about Meta-learning. 
However, there is no tutorial systematically reviewing relevant works at ACL/EMNLP/NAACL/EACL/COLING.



\section{Tutorial Structure and Content}
A typical machine learning algorithm, e.g., deep learning, can be considered as a sophisticated function. 
The function takes training data as input and a trained model as output. 
Today the learning algorithms are mostly human-designed. 
These algorithms have already achieved significant progress towards artificial intelligence, but still far from optimal. 
Usually, these algorithms are designed for one specific task and need a lot of labeled training data.
One possible method that could overcome these challenges is meta-learning, also known as ‘Learning to Learn’, which aims to learn the learning algorithm. 
In the image processing research community, meta-learning has shown to be successful, especially few-shot learning. 
It has recently also been widely adopted to a wide range of NLP applications, which usually suffer from data scarcity. 
This tutorial has two parts.
In part I, we will introduce several meta-learning approaches (\textbf{estimated 1.5 hours}).
In part II, we will highlight the applications of the meta-learning methods to NLP (\textbf{estimated 1.5 hours}). 

\subsection{Part I - Introduction of Meta Learning}
We will start with the problem definition of meta-learning, and then introduce the most well-known meta-learning approaches below.

\subsubsection{Learning to Initialize}
Gradient descent is the core learning algorithm for deep learning. Most of the components in gradient descent are handcrafted. First, we have to determine how to initialize network parameters. Then the gradient is computed to update the parameters, and the learning rates are determined heuristically. 
Determining these components usually need experience, intuition, and trial and error. 
With meta-learning, those hyperparameters can be learned from data automatically.
  Among these series of approaches, learning a set of parameters to initialize gradient descent, or learning to initialize, is already widely studied. 
  
  Column (A) of Table~\ref{table:ref} lists the NLP papers using learning to initialize.
  Learning to initialize is the most widely applied meta-learning approach in NLP today. 
  The idea of learning to initialize spreads quickly in NLP probably because the idea of looking for better initialization is already widespread before the development of meta-learning. 
  The researchers of NLP have applied lots of different transfer learning techniques to find a set of good initialization parameters for a specific task from its related tasks. 
  Here we will not only introduce learning to initialize but also compare its difference with typical transfer learning.
  
 \subsubsection{Learning to Compare}
Besides the gradient descent-based learning algorithm, the testing examples’ labels are determined by their similarity to the training examples in some learning algorithms. 
In this category, methods to compute the distance between two data points are crucial. Therefore, a series of approaches have been proposed to learn the distance measures for the learning algorithms. 
This category of approaches is also known as metric-based approaches. 

Column (B) of Table~\ref{table:ref} lists the NLP papers using learning to compare.
Natural language is intrinsically represented as sophisticated sequences. 
Comparing the similarity of two sequences is not trivial, and widely used handcrafted measures, such as, Euclidean distance, cannot be directly applied, which motivates the research of learning to compare in NLP. 

 
   \subsubsection{Other Methods}
   Although the above two methods dominate the NLP field at the moment, other meta-learning approaches have also shown their potential. 
   For example, besides parameter initialization, other gradient descent components such as learning rates and network structures can also be learned.
In addition to learning the components in the existing learning algorithm, some attempts even make the machine invent an entirely new learning algorithm beyond gradient descent.
There is already some effort towards learning a function that directly takes training data as input and outputs network parameters for the target task. 
Column (C) of Table~\ref{table:ref} lists these methods.


\subsection{Part II - Applications to NLP tasks}
There is a growing number of studies applying meta-learning techniques to NLP applications and achieving excellent results. In the second part of the tutorial, we will review these studies. Here we summarize these studies by categorizing their applications. Please refer to Table~\ref{table:ref} for a detailed list of studies we plan to cover in the tutorial. 


\subsubsection{Text Classification}
Text classification has a vast spectrum of applications, such as sentiment classification and intent classification. 
The meta-learning algorithms developed for image classification can be applied to text classification with slight modification to incorporate domain knowledge in each application~\cite{Yu:ACL18,Tan:EMNLP19,Geng:EMNLP19,Sun:EMNLP19,Dou:EMNLP19,Bansal:arXiv19}. 


\subsubsection{Sequence Labeling}
Using a meta-learning algorithm to make the model fast adapt to new languages or domains is also useful for sequence labeling like name-entity recognition (NER)~\cite{Wu:AAAI20} and slot tagging~\cite{Hou:ACL20}.
However, the typical meta-learning methods developed on image classification may not be optimal for sequence labeling because sequence labeling benefits from modeling the dependencies between labels, which is not leveraged in typical meta-learning methods. Techniques, such as the collapsing labeling mechanism, are proposed to optimize meta-learning for sequence labeling problem~\cite{Hou:ACL20}.

\subsubsection{Automatic Speech Recognition and Neural Machine Translation}
Automatic speech recognition (ASR), Neural machine translation (NMT), and speech translation require a large amount of labeled training data. Collecting such data is cost-prohibitive. To facilitate the expansion of such systems to new use cases, 
meta-learning is applied in these systems for the fast adaptation to new languages in NMT~\cite{Gu:EMNLP18} and 
ASR~\cite{Hsu:ICASSP20,Chen:INTERSPEECH20}, and fast adaptation to new accents~\cite{Winata:INTERSPEECH2020}, new speakers~\cite{Klejch:ASRU19,Klejch:INTERSPEECH18}, code-switching~\cite{Winata:ACL2020} in ASR. 


\subsubsection{Relation Classification and Knowledge Graph Completion}
The typical supervised learning approaches for relation classification and link prediction for knowledge graph completion require a large number of training instances for each relation. 
However, only about 10\% of relations in Wikidata have no more than ten triples~\cite{Vrandei:ACM14}, so many long-tail relations suffer from data sparsity. 
Therefore, meta-learning has been applied to the relation classification and knowledge graph completion to improve the performance of the relations with limited training examples~\cite{Obamuyide:ACL19,Bose:arXiv19,Lv:EMNLP19,Wang:EMNLP19,Ye:ACL19,Chen:EMNLP19,Xiong:EMNLP18,Gao:AAAI19}.

\subsubsection{Task-oriented Dialogue and Chatbot}
Domain adaptation is an essential task in dialog system building because modern personal assistants, such as Alexa and Siri, are composed of thousands of single-domain task-oriented dialog systems.
However, training a learnable model for a task requires a large amount of labeled in-domain data, and collecting and annotating training data for the tasks is costly since it involves real user interactions.
Therefore, researchers apply meta-learning to learn from multiple rich-resource tasks and adapt the meta-learned models to new domains with minimal training samples for dialog response generation~\cite{Qian:ACL19} and dialogue state tracking (DST)~\cite{Huang:ACL20}. 

Also, training personalized chatbot that can mimic speakers with different personas is useful but challenging. 
Collecting many dialogs involving a specific persona is expensive, while it is challenging to capture a persona using only a few conversations. Thus, meta-learning comes into play for learning persona with few-shot example conversations~\cite{Madotto:ACL19}.

%\item More applications: Question answering (QA), Semantic Parsing
%QA: Multi-source Meta Transfer for Low Resource Multiple-Choice Question Answering, ACL 2020
% Po-Sen Huang, Chenglong Wang, Rishabh Singh, Wen-tau Yih, Xiaodong He, Natural Language to Structured Query Generation via Meta-Learning, NAACL 2018 %Lee: what is this? 
%semantic parsing: Daya Guo, Duyu Tang, Nan Duan, Ming Zhou, Jian Yin, Coupling Retrieval and Meta-Learning for Context-Dependent Semantic Parsing, ACL, 2019
% Lee: Actually, the use of meta learning in the above two papers is to "personalized" model, which is different from other papers


\section{Reading list}
We encourage the audience to read the papers of some well-known meta-learning techqnieus before the tutorial, which are listed below.
\begin{itemize}
\item Learning to Initialize~\cite{Finn:ICML17}
\item Learning to Compare~\cite{Snell:NIPS17,Vinyals:NIPS16}
\item Other Methods~\cite{Ravi:ICLR17,Andrychowicz:NIPS16}
\end{itemize}




\begin{comment}

\section{Deprecated outlines}
  %  \item Application of methods to (NLP) tasks
  %  \begin{itemize}
  %      \item Taxonomy of methods vs. problems (any correlation? why method type A is common in problem B)
  %      \item Available datasets and results
  %  \end{itemize}
  %  \item Application of methods to use cases (e.g., language transferring, domain transferring, faster adaptation, zero-/few- shot learning, supervised learning with rich resources)
%    \begin{itemize}
   %     \item Taxonomy of methods vs. use cases (any correlation?)
 %       \item Ways of buidling meta-training / meta-testing split
  %  \end{itemize}
  %  \item Relation between meta-learning and other techniques
  %  \item Potential future direction?


%\begin{table*}[tb!]
%\centering
%\caption{Data efficiency vs. meta-learning methods. ZS: zero-shot; FS: few-shot.}
%\label{table:data-efficiency}
%  \resizebox{2\columnwidth}{!}{
%    \begin{tabular}{|l||l|l|l|l|}
%      \hline
%      & ZS / FS domain transferring &  ZS / FS language transferring &  ZS / FS task transferring & Others \\ \hline\hline
%      Learning to initialize & & & & \\ \hline
%      Learning to initialize & & & & \\ \hline
%      Learning to compare & & & & \\ \hline
%      Neural network search & & & & \\ \hline
%      Learning to optimize & & & & \\ \hline
%      Learning the learning algorithm & & & & \\ \hline
%      Learning to select data & & & & \\ \hline
%      Others & & & & \\ \hline
%    \end{tabular}
%  }
%\end{table*}

%\begin{table*}[tb!]
%\centering
%\caption{Generalizability vs. meta-learning methods.}
%\label{table:generalizability}
%  \resizebox{2\columnwidth}{!}{
%    \begin{tabular}{|l||l|l|l|l|l|}
%      \hline
%      & \tabincell{l}{Transferring learning (domain/\\language/task), ZS/FS in target} & \tabincell{l}{Transferring learning (domain/\\language/task), rich resource in target} & Lifelong learning & \tabincell{l}{Generalizability across training/test\\ split (usually single domain)} & Others \\ \hline\hline
%      Learning to initialize & & & & & \\ \hline
%      Learning to initialize & & & & & \\ \hline
%      Learning to compare & & & & & \\ \hline
%      Neural network search & & & & & \\ \hline
%      Learning to optimize & & & & & \\ \hline
%      Learning the learning algorithm & & & & & \\ \hline
%      Learning to select data & & & & & \\ \hline
%      Others & & & & & \\ \hline
%    \end{tabular}
%  }
%\end{table*}

%\begin{table*}[tb!]
%\centering
%\caption{Other benefits vs. meta-learning methods. }
%\label{table:generalizability}
%  \resizebox{2\columnwidth}{!}{
%    \begin{tabular}{|l||l|l|l|}
%      \hline
%      & \tabincell{l}{Model accuracy in test split \\ (usually single domain with full supervision)} & \tabincell{l}{Computation/memory/storage efficiency\\ (runtime, training?)} & Others \\ \hline\hline
%      Learning to initialize & & & \\ \hline
%      Learning to initialize & & & \\ \hline
%      Learning to compare & & & \\ \hline
%      Neural network search & & & \\ \hline
%      Learning to optimize & & & \\ \hline
%      Learning the learning algorithm & & & \\ \hline
%      Learning to select data & & & \\ \hline
%      Others & & & \\ \hline
%    \end{tabular}
%  }
%\end{table*}

\section{Breadth}
In the tutorial, we will review classic and novel meta-learning algorithms as well as discuss representative works of applying meta-learning to popular NLP problems. Breadth and coverage of algorithms and works are one of the main focuses of the tutorial. We will spend less than 20\% of the time in the works from the presenters.

\section{Diversity}
The speakers comprise researchers from Asia, Europe, and North America. They come from both academia and industry to provide a balanced viewpoint. They also vary in the seniority, from young scientists to senior researchers with abundant experience in teaching. Meta-learning itself also benefits diversity. 
As one of the main applications of the meta-learning approaches is to find better metrics, model architectures, or initializations such that the meta-trained model can generalize well in new tasks with limited data, the approach is often used at efficient knowledge transferring between domains and languages, and has seen many promising results. 
Meta-learning has the potential to democratize the progress of machine learning and NLP for different domains, languages, and countries in a scalable way.

\section{Tutorial Logistics}
\begin{itemize}
\item Duration: 3 hours
 \item Description of Presentation format: presented by three speakers
 \item Specification of any prerequisites for the attendees: understand derivatives as found in introductory Calculus; understand basic machine learning concepts such as classification, model optimization, and gradient descent
 \item Venue preference: we do not have any preference and we are happy to present on any of the venues (EACL/NAACL-HLT/ACL-IJCNLP/EMNLP)
 \item Special equipment required for the tutorial: none
 \item Open access: we agree to allow the publication of our slides and video recording of the tutorial in the ACL Anthology, and we will make other teaching materials (e.g., data, sample code) available online
\end{itemize}

\section{Intended Audience}
This tutorial will benefit a wide range of audiences. The tutorial contains sufficient introductory meta-learning materials to let audiences who are not familiar with this technology to understand its fundamental concept and theory. However, we expect that the audiences already have some background knowledge about machine learning. We will review some up-to-date research directions of applying meta-learning to NLP, so the audiences who already have experience in meta-learning can still learn how to apply the approach to different realistic NLP problems. 
Based on the tutorial content and the feedback from INTERSPEECH, where we will give a talk on a similar topic, we believe that this tutorial will attract a lot of audiences interested in this new technology. 
The estimated number of participants is 200.

\section{Tutoral Experience of Presenters}

\begin{itemize}
\item The speakers gave a tutorial on a similar topic (Meta Learning and its applications to Human Language Processing) at INTERSPEECH 2020\footnote{\url{http://www.interspeech2020.org/Program/Tutorials/}}.
\item The speakers are in the organization committee of an ACL 2021 workshop on a similar topic (Meta Learning and Its Applications to Natural Language Processing).
\begin{itemize}
\item Organization Committee of the workshop: Hung-yi Lee, Mitra Mohtarami, Shang-Wen Li, Di Jin, Mandy Korpusik, Annie Dong, Ngoc Thang Vu, Dilek Hakkani-Tur
\end{itemize}
\item Hung-yi Lee gave the tutorial entitled Generative Adversarial Network and its Applications to Signal Processing and Natural Language Processing at ICASSP 2018, APSIPA 2018, ISCSLP 2018, and INTERSPEECH 2019.
\begin{itemize}
\item This tutorial has the most participants among the 14 tutorials in ICASSP 2018.
\item This tutorial has the most participants among the 8 tutorials in INTERSPEECH 2019.
\end{itemize}
\item Hung-yi Lee has taught Meta Learning in the machine learning course at National Taiwan University. The recording of the lectures can be found on YouTube and it has seen more than 100k views.
\item Ngoc Thang Vu has taught Meta Learning in his machine learning courses (both theory and practical courses) at the Stuttgart University.
\end{itemize}

\section{Appendices}
\label{sec:appendix}
Appendices are material that can be read, and include lemmas, formulas, proofs, and tables that are not critical to the reading and understanding of the paper. 
Appendices should be \textbf{uploaded as supplementary material} when submitting the paper for review.
Upon acceptance, the appendices come after the references, as shown here.

\paragraph{\LaTeX-specific details:}
Use {\small\verb|\appendix|} before any appendix section to switch the section numbering over to letters.


\section{Supplemental Material}
\label{sec:supplemental}
Submissions may include non-readable supplementary material used in the work and described in the paper.
Any accompanying software and/or data should include licenses and documentation of research review as appropriate.
Supplementary material may report preprocessing decisions, model parameters, and other details necessary for the replication of the experiments reported in the paper.
Seemingly small preprocessing decisions can sometimes make a large difference in performance, so it is crucial to record such decisions to precisely characterize state-of-the-art methods. 

Nonetheless, supplementary material should be supplementary (rather than central) to the paper.
\textbf{Submissions that misuse the supplementary material may be rejected without review.}
Supplementary material may include explanations or details of proofs or derivations that do not fit into the paper, lists of
features or feature templates, sample inputs and outputs for a system, pseudo-code or source code, and data.
(Source code and data should be separate uploads, rather than part of the paper).

The paper should not rely on the supplementary material: while the paper may refer to and cite the supplementary material and the supplementary material will be available to the reviewers, they will not be asked to review the supplementary material.

\section{Biographies of Presenters}
%* The names, affiliations, email addresses and websites of the tutorial presenters, including a one-paragraph statement of their research interests, areas of expertise and experience in teaching for an international audience.

\textbf{Hung-yi Lee}\footnote{\url{https://speech.ee.ntu.edu.tw/~tlkagk/}} received the M.S. and Ph.D. degrees from National Taiwan University (NTU), Taipei, Taiwan, in 2010 and 2012, respectively. From September 2012 to August 2013, he was a postdoctoral fellow in Research Center for Information Technology Innovation, Academia Sinica. From September 2013 to July 2014, he was a visiting scientist at the Spoken Language Systems Group of MIT Computer Science and Artificial Intelligence Laboratory (CSAIL). He is currently an associate professor of the Department of Electrical Engineering of National Taiwan University, with a joint appointment at the Department of Computer Science & Information Engineering of the university. His research focuses on machine learning (especially deep learning), speech processing and natural language processing. He owns a YouTube channel teaching deep learning (in Mandarin) with more than \textbf{5M} views and \textbf{60k} subscribers. 

\textbf{Ngoc Thang Vu}\footnote{\url{https://www.ims.uni-stuttgart.de/en/institute/team/Vu-00002}} received his Diploma (2009) and PhD (2014) degrees in computer science from Karlsruhe Institute of Technology, Germany. From 2014 to 2015, he worked at Nuance Communications as a senior research scientist and at Ludwig-Maximilian University Munich as an acting professor in computational linguistics. In 2015, he was appointed assistant professor at University of Stuttgart, Germany. Since 2018, he has been a full professor at the Institute for Natural Language Processing in Stuttgart. His main research interests are natural language processing (esp. speech recognition and dialog systems) and machine learning (esp. deep learning) for low-resource settings.

\textbf{Shang-Wen Li}\footnote{\url{https://scholar.google.com/citations?user=wFI97HUAAAAJ}} is a senior Applied Scientist at Amazon AI. His research focuses on spoken language understanding, dialog management, and natural language generation. His recent interest is transfer learning for low-resourced conversational bots. He earned his Ph.D. from MIT Computer Science and Artificial Intelligence Laboratory (CSAIL) in 2016. He received M.S. and B.S. from National Taiwan University. Before joining Amazon, he also worked at Apple Siri researching conversational AI.

%For a more detailed list of related works, please refer to our webpage of the INTERSPEECH 2020 special session - Meta Learning for Human Language Technology\footnote{https://sunprinces.github.io/interspeech2020-meta-learning/}.

%The presenters will publish (or submit) the following papers related to meta learning:
%Jui-Yang Hsu, Yuan-Jui Chen, Hung-yi Lee, Meta Learning for End-to-End Low-Resource Speech Recognition, ICASSP 2020 
%Shang-Wen Li, Jason Krone, and Yi Zhang, Meta learning to classify intent and slot labels with perturbed few shot examples, submitted to SLT 2021
%Hongyin Luo, Shang-Wen Li, and James Glass, Medical dialog planning with few shot noisy examples with Meta learning, INTERSPEECH 2020
%Yi-Chen Chen, Jui-Yang Hsu, Hung-yi Lee, Network Architecture Search with Meta Learning for End-to-End Low-Resource Speech Recognition, will to submit to INTERSPEECH 2020
%Sung-Feng Huang, Jui-Yang Hsu, Hung-yi Lee, What does MAML learn in Low-Resource Speech Recognition?, will to submit to INTERSPEECH 2020
%Pavel Denisov, Ngoc Thang Vu, Few-shot Learning for Intent Recognition on Speech, will to submit to INTERSPEECH 2020
%Cennet Oguz, Ngoc Thang Vu, Concept Tagging for New Domains with Meta Learning, will to submit to INTERSPEECH 2020

\end{comment}
